User-in-the-loop Evaluation of Multimodal LLMs for Activity Assistance

Our research investigates the capability of modern multimodal reasoning models, powered by Large Language Models (LLMs), to facilitate vision-powered assistants for multi-step daily activities. Such assistants must be able to 1) encode relevant visual history from the assistant's sensors, e.g., camera, 2) forecast future actions for accomplishing the activity, and 3) replan based on the user in the loop. To evaluate the first two capabilities, grounding visual history and forecasting in short and long horizons, we conduct benchmarking of two prominent classes of multimodal LLM approaches -- Socratic Models and Vision Conditioned Language Models (VCLMs) on video-based action anticipation tasks using offline datasets. These offline benchmarks, however, do not allow us to close the loop with the user, which is essential to evaluate the replanning capabilities and measure successful activity completion in assistive scenarios. To that end, we conduct a first-of-its-kind user study, with 18 participants performing 3 different multi-step cooking activities while wearing an egocentric observation device called Aria and following assistance from multimodal LLMs. We find that the Socratic approach outperforms VCLMs in both offline and online settings. We further highlight how grounding long visual history, common in activity assistance, remains challenging in current models, especially for VCLMs, and demonstrate that offline metrics do not indicate online performance.

==> sec/3_method.tex <==
\section{Offline Benchmarks}
\label{sec:offline_benchmarks}
Our goal is to make progress toward vision-powered assistants that can reason about their user's context such as the user's progress in a daily activity from visual sensors and provide relevant recommendations on future actions. Various action anticipation benchmarks previously proposed by the research community also require such reasoning capabilities. Therefore, we choose them to evaluate SOTA multimodal LLM approaches. 

\subsection{Benchmark Tasks}
% While a plethora of video-based action anticipation benchmarks exist~\cite{nagarajan2020ego}, we choose three representative ones such that they cover the space of short to long visual history and short to long forecasting horizon. Specifically, we choose Short-term action Anticipation (STA) benchmark proposed by EpicKitchens (EK-55) dataset~\cite{epickitchen21}, Long-term action Anticipation (LTA) from Ego4D~\cite{ego4d}, and Visual Planning for Assistance (VPA) task on CrossTask dataset from~\cite{patel2023pretrained}. As summarized in Table~\ref{tab:offline_benchmarks}, STA requires grounding a short history -- 1 second video for short horizon prediction (single next action), while LTA focuses on predicting a sequence of 20 future actions after grounding long untrimmed visual history corresponding to approximately 8 or more actions. In comparison to LTA and STA, VPA on CrossTask operates on medium-range untrimmed visual history corresponding to 3-4 actions for medium horizon forecasting of 3-4 future actions. The output is mapped to a closed set of verbs, nouns, and actions i.e., (verb, noun) pairs in each benchmark. We use the same evaluation metrics as were proposed by the original benchmarks for consistency with prior work. Consequently, STA is evaluated using top-5 verb, noun, action mean classification accuracy, LTA is evaluated using edit distance, and VPA is evaluated with order-agnostic mean intersection over union (mIoU) and a strict order-respecting metric called Success rate metrics (defined as in~\cite{patel2023pretrained}).
While a plethora of video-based action anticipation benchmarks exist~\cite{nagarajan2020ego}, we choose two representative ones such that they cover the space of medium to long visual history and medium to long forecasting horizon -- the settings closest to activity assistance in real-world vision-powered systems\footnote{We exclude anticipation benchmarks like EpickKitchens~\cite{epickitchen21} as they consider short visual histories (1s) and are not aligned with real-world activity assistance.}
% Given our focus on real-world activity assistance, we do not consider other popular video action anticipation benchmarks such as EpicKitchens~\cite{epickitchen21} that consider only short visual history of 1 sec.}. 
Specifically, we choose Long-term action Anticipation (LTA) from Ego4D~\cite{ego4d}, and Visual Planning for Assistance (VPA) task on the CrossTask dataset from~\cite{patel2023pretrained}. As summarized in Table~\ref{tab:offline_benchmarks}, LTA focuses on predicting a sequence of future actions 
% \footnote{3542 actions in the table is the feasible actions from Ego4D train set}  
with a length of $Z=20$ after grounding a long untrimmed visual history corresponding to approximately 8 or more actions. Compared to LTA, VPA on CrossTask operates on a medium-range untrimmed visual history corresponding to 3-4 actions for medium-horizon forecasting of $Z=3\sim4$ future actions.\change{While not part of the original benchmark, we also look at LTA with $Z=5$ to help disambiguate the challenges of long-history and long-horizon in prediction.} The output is mapped to a closed set of verbs, nouns, and actions i.e., (verb, noun) pairs in each benchmark. We use the same evaluation metrics as were proposed by the original benchmarks for consistency with prior work. The predicted action sequences in LTA are evaluated using the edit distance. VPA is evaluated with action prediction accuracy at each step (mean accuracy), order-agnostic mean Intersection over Union (mIoU), and a strict order-respecting metric Success Rate for the predicted sequence (defined as in~\cite{patel2023pretrained}).

% \bc{add VCLM, socratic description and details}

% no finetuning on training and testing
% pretraining+ in context prompt



\subsection{Multimodal LLMs}
\label{sec:offline_mm_llm}
All our benchmarks require grounding information from untrimmed video history for future action prediction. If the visual history is appropriately represented, the future action prediction task can be framed as a sentence completion task using an LLM~\cite{llama,llama2}. We evaluate two predominant approaches to representing visual history for such reasoning with LLMs to predict future actions. 
 
\noindent\textbf{Socratic model.} The main idea behind the Socratic approach is to \change{use pretrained vision-language models (VLMs) to} convert non-textual modalities into text for a downstream LLM. One could represent different task-relevant information from the untrimmed video history as text such as objects, actions, and open-set narrations describing the events in the video. We find that such narrations tend to be a superset of various contextual information that could be extracted from video, including objects and actions. Appendix~\ref{sub_additional_ex} provides this quantitative comparison for LTA.  Instead of using objects, actions, and narrations, we therefore choose only narrations from a video narration model to represent visual history as text in our Socratic models, akin to various existing works~\cite{huang2023palm,socratic}. 

\noindent\textbf{Vision-conditioned language models (VCLMs).} These models embed the visual modality as continuous tokens that can be concatenated with text tokens and then passed as input to an LLM. A linear~\cite{llava, moon2023anymal} or a non-linear projection layer~\cite{patel2023pretrained} is fine-tuned to align these continuous tokens with the embedding space of text tokens for a given LLM. Thus, \change{unlike Socratic Models, VCLMs can process both embedded visual information and text.}  

% Since these models are capable of processing only a limited number of frames\footnote{SOTA models such as AnyMAL process only 8 frames of video irrespective of its length. Typical videos in our benchmarks require grounding on average $>$500 frames corresponding to multiple task-relevant steps.}, which is insufficient for video tasks requiring grounding of long visual history -- we leverage both text and continuous embeddings to encode the visual history in our VCLMs \change{and evaluate the contribution of the additional implicit visual encoding that VCLMs provide}. 

\change{In contrast to VCLMs used for image captioning and VQA tasks, where visual information is only encoded using the continuous embeddings~\cite{flamingo}, we choose to use both continuous embeddings as well as text tokens for encoding visual history in our benchmark tasks. Visual encoders in current SOTA VCLMs use limited and uniformly-sampled frames from input videos for video tasks. For instance, AnyMAL processes only 8 frames of video irrespective of its length~\cite{moon2023anymal}. However, typical videos in our benchmarks require grounding on average $>$500 frames corresponding to multiple task-relevant steps. 
% Consequently,  we leverage both text and continuous embeddings to encode the visual history in our VCLMs and evaluate the contribution of the additional implicit visual encoding that VCLMs provide.
To better capture such long visual histories, we thus leverage both text tokens and continuous embeddings to encode the visual history in our VCLMs.}
% we encode visual history via text using the same VLMs from the Socratic model in addition to continuous visual embeddings. Thus our VCLMs models measure the benefit of continuous visual history in addition to text-based visual history.}
Appendix~\ref{sub_additional_ex} shows an ablation comparing VCLMs that only use continuous embeddings for the encoding history with those that use both continuous embeddings and text tokens in LTA. 



% This approach provide an alternative approach to combining pre-trained models for new downstream tasks. This framework does not require training, but instead uses language as a medium for communication between the models. This is distinct from other multimodal approaches, such as training a single model over all modalities, and may be used in conjunction with them. In our experiments, we use Lavila \cite{zhao2023lavila} trained on Ego4D egocentric videos \cite{grauman2022ego4d} as the video captioning model to transfer video information to text. In addition, the next action prediction task becomes the text completion task to generate the future text sequence. We use the instruction-tuned LLaMA2 13/70B \cite{touvron2023llama} for text completion.
%\bc{talk about lavila captions}
% \textbf{Prompts for in-context learning}:

 % We have formulated the action anticipation task as a sentence completion task and have predicted future actions by prompting large language models (LLMs) with past action descriptions. Out-of-the-box large-language models do not work well in the action anticipation task in a zero-shot setting. Following the usual practice, we have designed the prompt with a few examples to maximize the reference given to the model. The template of our prompts consists of an instruction, a few examples, followed by a query. The instruction is to adapt the model to the future action prediction task. Each example contains $N$ full-sentence narrations or the corresponding $N$ action labels of a verb or verb-noun pair. We also provide the future $M$ actions in the examples. Similarly, the query is composed of narrations or action labels of the past $N^\prime$ actions. We used a larger number of action observations $N^\prime > N $ in the query. Different prompt templates for each task are shown in the supplement section \ref{sup:prompt_template}.

% \noindent \textbf{Narrations or action labels:} 
% Socratic Models (SMs) have demonstrated that large pre-trained models can be combined through language (by prompting) without the need for training, to carry out new downstream multimodal tasks.
% The idea is to use a video captioning model (lavila) or segmentation model (VideoCLIP) to capture the action context, providing more information related to the visual input. %
% To do so, we use the given action segments and generate a caption or action label from each past action. 

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=.63\columnwidth]{figures/socratic.png}
%     \caption{
%      Socratic Inference. \bc{place holder}
%     }
%     \label{fig:diagram}
% \end{figure}


%\end{wrapfigure}

\subsection{Experiment Setup}
\label{sec:experiment_setup}

% \noindent \textbf{Pre-training}: We obtain multimodal understanding capabilities by pre-training a lightweight adapter for each modality to project the input signals into the text token embedding space of a specific LLM (Figure \ref{fig:diagram}). This creates a joint token embedding space, with tokens representing either text or video. The number of token embeddings used to represent each input modality is set to 64. The parameters of the underlying LLM are frozen during the alignment training, which allows it to reach convergence faster than training end-to-end from scratch and to inherit the reasoning capabilities of the LLM at inference time. For each text caption and video segment pair $(\mathbf{X}_{\texttt{text}}, \mathbf{X}_{\texttt{modality}})$, we align them using the Perceiver Resampler \cite{flamingo} for vision encoder.
%
% \vspace{-5pt}
% \begin{align}
%     p(\mathbf{X}_{\texttt{text}} | \mathbf{X}_{\texttt{modality}}) = \prod_{i=1}^{L} p_{\theta}(\mathbf{X}^{[i]}_{\texttt{text}} | \mathbf{Z}_{\texttt{modality}}, \mathbf{Z}^{[1:i\small{-}1]}_{\texttt{text}}) \\
%     \mathbf{Z}_{\texttt{modality}} = \texttt{Projection}_{\theta}(h_{\texttt{latents}}, g(\mathbf{X}_{\texttt{modality}}))
% \end{align}

% \noindent \textbf{Datasets}:
% For video alignment, we trained with HowTo100M Auto-Aligned (HTM-AA) \cite{han2022temporal}. For the video encoder, we use Intern video \cite{wang2022internvideo}. We follow the same instruction-tuned LLaMA2 13/70B \cite{touvron2023llama} for the text model.

% \noindent \textbf{In context prompt}:
% Similar to the inferencing of socratic model using incontext prompt as in section \ref{subsec:methods:Socratic}, we also input the previous video segment as visual history. 





==> tables/EK55.tex <==
\begin{table}[t]
\centering
\scriptsize
\begin{tabular}{lccccc}
\multicolumn{1}{l|}{Method} & \multicolumn{1}{c|}{Modality} & Prompt & Visual feature      & verb & noun   \\ \hline
% \multicolumn{1}{l|}{Socratic 13B} & \multicolumn{1}{c|}{T}   & Caption  &    &         \\
% \multicolumn{1}{l|}{VCLM 13B} & \multicolumn{1}{c|}{V+T}  &  Caption  & Internvideo   & 13.5       \\
% \hline
\multicolumn{1}{l|}{Socratic 13B} & \multicolumn{1}{c|}{T}   &  GT action &    & 13.2   &  15.8  \\
\multicolumn{1}{l|}{Socratic 70B} & \multicolumn{1}{c|}{T}   &  GT action &    & 14.2  &     \\
\multicolumn{1}{l|}{VCLM 13B} & \multicolumn{1}{c|}{V+T}  &   GT action & Internvideo   & 14.9   &    \\
\multicolumn{1}{l|}{VCLM 70B} & \multicolumn{1}{c|}{V+T}  &   GT action & Internvideo   &  \textbf{15.5} &    \\
\hline
\end{tabular}
\caption{\textbf{Next action prediction on the EK-55. }
}
\label{tab:ek55}
\end{table}


==> tables/LTA_Z5.tex <==
%\begin{table}[t]
\begin{wraptable}{r}{5.0cm}
\centering
\scriptsize
\resizebox{!}{0.8cm}{
\begin{tabular}{crrr}
\hline
\textbf{Model}        & (Z=5)Verb  & Noun  & Action \\ \hline
Socratic 13B & 0.689 & 0.681 & 0.919 \\
VCLM 13B     & 0.696 & 0.669 & 0.923 \\
Socratic 70B & \textbf{0.683} & \textbf{0.661} & \textbf{0.917}  \\
VCLM 70B     & 0.696 & 0.669 & 0.923  \\ \hline
\end{tabular}}
\caption{Long-term action anticipation on Ego4D Z=5.}
\vspace{-0.2cm}
\label{tab:long_term_results_z5}
%\end{table}
\end{wraptable}


==> tables/aria.tex <==
\begin{table}[t]
\centering
\scriptsize
\begin{tabular}{lccc}
\multicolumn{1}{l|}{Method} & \multicolumn{1}{c|}{Modality}  & Visual feature      & BERT score   \\ \hline
\multicolumn{1}{l|}{Socratic 13B} & \multicolumn{1}{c|}{T}      &    & 0.508       \\
\multicolumn{1}{l|}{VCLM  13B} & \multicolumn{1}{c|}{V+T}      & Internvideo  & 0.526       \\
\multicolumn{1}{l|}{Socratic 70B} & \multicolumn{1}{c|}{T}      &    & 0.516       \\
\multicolumn{1}{l|}{VCLM  70B} & \multicolumn{1}{c|}{V+T}      & Internvideo  & \textbf{0.528}       \\
\hline
\end{tabular}
\caption{\textbf{Next action caption prediction on the Aria data.}
}
\label{tab:aria}
\end{table}


==> tables/lta.tex <==
\begin{table}[h]
\centering
\scriptsize
\resizebox{\columnwidth}{!}{
\begin{tabular}{lccclll}
\toprule
\multirow{2}{*}{\textbf{Model}} &\multirow{2}{*}{\textbf{Visual History}}  & \multirow{2}{*}{\textbf{Visual Encoder}}  &   \multicolumn{3}{c}{ED@(Z=20)$\downarrow$}  \\ 
\cmidrule(l){4-6} 
 &    &  & Verb   & Noun    & Action \\ \midrule
\multicolumn{1}{l}{AntGPT\cite{zhao2023antgpt}} & T  & CLIP & 0.756  & 0.725   & -       \\ 
% \multicolumn{1}{l}{Palm \cite{huang2023palm}} && T  &  & \textbf{0.695}  & \textbf{0.650}   & \textbf{0.885}    \\ 
\multicolumn{1}{l}{Palm*\tablefootnote{We include Palm$^*$ as the reproduced version of Palm~\cite{huang2023palm}.} \cite{huang2023palm}}&  T  & Blip2 & 0.732  & 0.812   & 0.958    \\ 
\multicolumn{1}{l}{Socratic 13B} & T  & LaViLa& 0.731 & 0.732     &   0.929      \\ 
\multicolumn{1}{l}{Socratic 70B} & T  &LaViLa& \textbf{0.726}   &   \textbf{0.712}  & \textbf{0.928}        \\ 
\midrule
%\multicolumn{1}{l}{VideoLLM \cite{chen2023videollm}}& & V+T  &  & 0.717  & 0.736   & 0.925    \\ 
\multicolumn{1}{l}{VCLM 13B} & V+T  & Internvideo+LaViLa &  0.740 &  0.751   &  0.932     \\ 
\multicolumn{1}{l}{VCLM 70B} & V+T  & Internvideo+LaViLa &  0.739 & 0.731   & 0.931      \\ 
%\multicolumn{1}{l}{ICVAE \cite{mascaro2022intention}} & V+T  &  & 0.741  & 0.739   & 0.930   not LLM   \\ 
\midrule
\multicolumn{1}{l}{\color{gray}{Ego4D (supervised) \cite{grauman2022ego4d}}} & \color{gray}{V} & \color{gray}{SlowFast}  & \color{gray}{0.745}  & \color{gray}{0.779}   & \color{gray}{0.941}       \\ 
\multicolumn{1}{l}{\color{gray}{VLaMP (supervised) \cite{patel2023pretrained}}}& \color{gray}{V+T}  & \color{gray}{S3D} & \color{gray}{0.730}  & \color{gray}{0.772}   & \color{gray}{0.932}    \\ 
\bottomrule
\end{tabular}}
\caption{\textbf{Long-term action anticipation on Ego4D.} Edit distance values for forecasting horizon of $Z=20$ actions is shown on v1 validation set.} %\bc{do we want to add the Z=5 results here? I think adding it in the supplement should be enough}
\vspace{-0.2cm}
\label{tab:long_term_results}
\end{table}

==> tables/rebuttal_adjacent_tab.tex <==
\begin{table}[]
\centering
\setlength{\tabcolsep}{3pt}
\resizebox{\columnwidth}{!}{%
% \begin{tabular}{c|r|rrr|rrr}
% \hline
% \textbf{Model}       & (Z=1) mAcc  & (Z=3) SR & mAcc & mIOU & (Z=4) SR & mAcc & mIOU \\ \hline
% Socratic 7B & 22.3       & 4.3     & 21.0 & 33.3 & 2.6     & 20.8 & 36.2 \\
% VCLM 7B     & \textbf{27.9}       & \textbf{6.8}     & \textbf{24.8} & \textbf{41.7} & \textbf{4.1}     & \textbf{24.0} & \textbf{45.0} \\ \hline
% \end{tabular}
\begin{tabular}{@{}cr|rrr|rrr@{}}
\toprule
  \multirow{2}{*}{\textbf{VPA Model}} &
  %\multirow{2}{*}{\textbf{ sample}} &
  $Z=1$ &
  \multicolumn{3}{c|}{$Z=3$} &
  \multicolumn{3}{c}{$Z=4$} \\ %\cmidrule(l){3-9} 
 &
  mAcc &
  SR &
  mAcc &
  mIOU &
  SR &
  mAcc &
  mIOU \\ \midrule
  Socratic 7B &
    22.3 &
     4.3 &
     21.0 &
     33.3 &
     2.6 &
    20.8 &
    36.2 \\
  VCLM 7B &
     \textbf{27.9} &
      \textbf{6.8} &
     \textbf{24.8} &
     \textbf{41.7} & 
     \textbf{4.1}  &
     \textbf{24.0} &
     \textbf{45.0} \\
  \bottomrule
\end{tabular}
\hspace{.3mm}
\vline
\hspace{.3mm}
\begin{tabular}{crrr}
\hline
\textbf{LTA Model}        & (Z=5)Verb  & Noun  & Action \\ \hline
Socratic 13B & 0.689 & 0.681 & 0.919 \\
VCLM 13B     & 0.696 & 0.669 & 0.923 \\
Socratic 70B & \textbf{0.683} & \textbf{0.661} & \textbf{0.917}  \\
VCLM 70B     & 0.696 & 0.669 & 0.923  \\ \hline
\end{tabular}
}
\vspace{-0.78cm}
\label{tab:vpa_7b}
\end{table}

==> tables/rebuttal_tab.tex <==
\begin{table}[]
\centering
\setlength{\tabcolsep}{3pt}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{crrrrrrrrrr}
\hline
\multirow{2}{*}{Model} & \multicolumn{3}{c}{LTA Z=5} & \multicolumn{1}{c}{VPA Z=1} & \multicolumn{3}{c}{VPA Z=3}                                                  & \multicolumn{3}{c}{VPA Z=4}                                                  \\ \cline{2-11} 
                       & Verb    & Noun    & Action  & \multicolumn{1}{l}{mAcc}    & \multicolumn{1}{l}{SR} & \multicolumn{1}{l}{mAcc} & \multicolumn{1}{l}{mIOU} & \multicolumn{1}{l}{SR} & \multicolumn{1}{l}{mAcc} & \multicolumn{1}{l}{mIOU} \\ \hline
Socratic 7B            &         &         &         & 22.3                        & 4.3                    & 21.0                     & 33.0                     & 2.6                    & 20.8                     & 36.2                     \\
VCLM 7B                &         &         &         & 27.9                        & 6.8                    & 24.8                     & 41.7                     & 4.1                    & 24.0                     & 45.0                     \\
Socratic 70B           & 0.683   & 0.661   & 0.917   &                             &                        &                          &                          &                        &                          &                          \\
VCLM 70B               & 0.696   & 0.669   & 0.923   &                             &                        &                          &                          &                        &                          &                          \\ \hline
\end{tabular}
}
\vspace{-0.7cm}
\label{tab:vpa_7b}
\end{table}

==> tables/vpa_7b_compressed.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
% \begin{table}[]
% \centering
% \setlength{\tabcolsep}{3pt}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{@{}llrrrrrrr@{}}
% \toprule
% \multirow{2}{*}{\textbf{Data}} &
%   \multirow{2}{*}{\textbf{Model}} &
%   $l=1$ &
%   \multicolumn{3}{c}{$l=3$} &
%   \multicolumn{3}{c}{$l=4$} \\ \cmidrule(l){3-9} 
%  &
%    &
%   \{n/m\}Acc &
%   SR &
%   mAcc &
%   mIOU &
%   SR &
%   mAcc &
%   mIOU \\ \midrule
% \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Cross-\\ task\end{tabular}} &
%   {Random} &
%   0.9   &
%   0.0   &
%   0.9   &
%   1.5   &
%   0.0   &
%   0.9   &
%   1.9  \\
%  &
%   VCLM &
%   29.0   &
%   7.0    &
%   25.8   &
%   41.1   &
%    2.8   &
%     22.9 &
%   42.9  \\
%  &
%   Socratic &
%    27.2   &
%   5.7     &
%    24.3   &
%    40.8   &
%   3.5    &
%   23.8   &
%   44.0   \\
%   \hline
%  &
%   \color{gray}{VLaMP (supervised)} &
%   \color{gray}{50.6} &
%   \color{gray}{10.3} &
%   \color{gray}{35.3} &
%   \color{gray}{44.0} &
%   \color{gray}{4.4} &
%   \color{gray}{31.7} &
%   \color{gray}{43.4} \\ 
%   \bottomrule
% \end{tabular}%
% }
% \caption{\textbf{Performance on CrossTask VPA. } }
% \label{tab:main-results-vlamp}
% \end{table}


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\centering
\setlength{\tabcolsep}{3pt}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|r|rrr|rrr}
\hline
\textbf{Model}       & (Z=1) mAcc  & (Z=3) SR & mAcc & mIOU & (Z=4) SR & mAcc & mIOU \\ \hline
Socratic 7B & 22.3       & 4.3     & 21.0 & 33.3 & 2.6     & 20.8 & 36.2 \\
VCLM 7B     & \textbf{27.9}       & \textbf{6.8}     & \textbf{24.8} & \textbf{41.7} & \textbf{4.1}     & \textbf{24.0} & \textbf{45.0} \\ \hline
\end{tabular}
}
\vspace{-0.7cm}
\label{tab:vpa_7b}
\end{table}

==> tables/vpa_7b_only.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
% \begin{table}[]
% \centering
% \setlength{\tabcolsep}{3pt}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{@{}llrrrrrrr@{}}
% \toprule
% \multirow{2}{*}{\textbf{Data}} &
%   \multirow{2}{*}{\textbf{Model}} &
%   $l=1$ &
%   \multicolumn{3}{c}{$l=3$} &
%   \multicolumn{3}{c}{$l=4$} \\ \cmidrule(l){3-9} 
%  &
%    &
%   \{n/m\}Acc &
%   SR &
%   mAcc &
%   mIOU &
%   SR &
%   mAcc &
%   mIOU \\ \midrule
% \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Cross-\\ task\end{tabular}} &
%   {Random} &
%   0.9   &
%   0.0   &
%   0.9   &
%   1.5   &
%   0.0   &
%   0.9   &
%   1.9  \\
%  &
%   VCLM &
%   29.0   &
%   7.0    &
%   25.8   &
%   41.1   &
%    2.8   &
%     22.9 &
%   42.9  \\
%  &
%   Socratic &
%    27.2   &
%   5.7     &
%    24.3   &
%    40.8   &
%   3.5    &
%   23.8   &
%   44.0   \\
%   \hline
%  &
%   \color{gray}{VLaMP (supervised)} &
%   \color{gray}{50.6} &
%   \color{gray}{10.3} &
%   \color{gray}{35.3} &
%   \color{gray}{44.0} &
%   \color{gray}{4.4} &
%   \color{gray}{31.7} &
%   \color{gray}{43.4} \\ 
%   \bottomrule
% \end{tabular}%
% }
% \caption{\textbf{Performance on CrossTask VPA. } }
% \label{tab:main-results-vlamp}
% \end{table}


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\centering
\setlength{\tabcolsep}{3pt}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}crrrrrrr@{}}
\toprule
  \multirow{2}{*}{\textbf{Model}} &
  %\multirow{2}{*}{\textbf{ sample}} &
  $Z=1$ &
  \multicolumn{3}{c}{$Z=3$} &
  \multicolumn{3}{c}{$Z=4$} \\ %\cmidrule(l){3-9} 
 &
  mAcc &
  SR &
  mAcc &
  mIOU &
  SR &
  mAcc &
  mIOU \\ \midrule
  Socratic 7B &
    22.3 &
     4.3 &
     21.0 &
     33.3 &
     2.6 &
    20.8 &
    36.2 \\
  VCLM 7B &
     \textbf{27.9} &
      \textbf{6.8} &
     \textbf{24.8} &
     \textbf{41.7} & 
     \textbf{4.1}  &
     \textbf{24.0} &
     \textbf{45.0} \\
  \bottomrule
\end{tabular}%
}
\vspace{-.8cm}
\label{tab:vpa}
\end{table}
